Enriching the NArabizi Treebank: A Multifaceted Approach to Supporting an Under-Resourced Language

In this paper we address the scarcity of annotated data for NArabizi, a Romanized form of North African Arabic used mostly on social media, which poses challenges for Natural Language Processing (NLP). We introduce an enriched version of NArabizi Treebank (Seddah et al., 2020) with three main contributions: the addition of two novel annotation layers (named entity recognition and offensive language detection) and a re-annotation of the tokenization, morpho-syntactic and syntactic layers that ensure annotation consistency. Our experimental results, using different tokenization schemes, showcase the value of our contributions and highlight the impact of working with non-gold tokenization for NER and dependency parsing. To facilitate future research, we make these annotations publicly available. Our enhanced NArabizi Treebank paves the way for creating sophisticated language models and NLP tools for this under-represented language.

==> Makefile <==
# set latexfile to the name of the main file without the .tex
#latexfile = eacltest
latexfile = acl2023
# put the names of figure files here.  include the .eps
figures = 

#includedfiles = Intro.tex State-of-the-art.tex Experiments.tex Discussion.tex
includedfiles = 


#Discussion.tex Intro_Djame.tex









#Algos.tex Discussion.tex Results.tex \
#	eacltest.tex experiences.tex intro.tex lexical-inpact.tex \
#	presentation-treebank.tex protocol.tex state-of-the-art-comparaison.tex\
#	corpus-setup-experiment.tex TODO.tex Tagset.tex crossparsing.tex \
#	new_intro.tex new_presTB.tex new_protocol.tex examples-marie.tex

TEX = pdflatex

# *.fig files may be in ./Figs
vpath %.fig Figs


all: pdf
$(latexfile).dvi : $(figures) $(includedfiles) $(latexfile).tex


%.eps : %.fig
	fig2dev -L eps $< > $@

$(latexfile).pdf : $(latexfile).tex $(includedfiles) $(figures)
	$(TEX)  $(latexfile).tex
#	$(TEX)  appendix.tex

pdf :	$(latexfile).tex
	$(TEX) $(latexfile).tex 

bib : $(latexfile).tex
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
#	bibtex $(latexfile)
#	$(TEX) $(latexfile)
#	$(TEX) $(latexfile)
#	$(TEX) $(latexfile)
	
	 
force:
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

appendix.pdf: 
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

	

$(latexfile).ps : $(latexfile).dvi
	dvips  -Ppdf $(latexfile) -o $(latexfile).ps

ps : $(latexfile).ps 

$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $(figures) $(latexfile).tex Figs/*.fig

tarball: $(latexfile).tar.gz


clean: 
	rm -f $(latexfile).bbl
	rm -f $(latexfile).log
	rm -f $(latexfile).dvi
	rm -f $(latexfile).blg
	rm -f $(latexfile).aux
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf
	rm -f $(latexfile).out
	
clean2:
	rm -f appendix.bbl
	rm -f appendix.log
	rm -f appendix.dvi
	rm -f appendix.blg
	rm -f appendix.aux
	rm -f appendix.ps
	rm -f appendix.pdf
		
check:
	cat $(latexfile).log | grep --text undef
	cat $(latexfile).log | grep --text multipl

dist-clean: clean
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf

viewX: pdf 
	open $(latexfile).pdf
	
viewA: pdf
	open -a Preview.app $(latexfile).pdf

view: $(latexfile).pdf
	open -a Skim.app $(latexfile).pdf
#	open -a Skim.app appendix.pdf 

gv: ps
	gv $(latexfile).pdf


edit: 
	xemacs $(latexfile).tex  & 


up:
	git pull

co:	commit
	
commit:
	git commit -m "update" 	./
	git push

commitsvn:
	svn commit -m "update" ./

upsvn:
	svn up

cp:
	cp $(latexfile).pdf /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/PapiersEnCours

ebib:
	open $(latexfile).bib


split: bib
	splitappendix $(latexfile).pdf 11
	open -a Skim.app submission.pdf appendix.pdf
	


==> raw_results_ner.tex <==

****************************************
Average results for model camembert+narabizi over 5 seeds:
  LOC:
    precision: 85.80
    recall: 85.60
    f1-score: 85.61
    support: 5000.00
  ORG:
    precision: 88.40
    recall: 56.77
    f1-score: 69.06
    support: 3100.00
  PER:
    precision: 67.26
    recall: 71.06
    f1-score: 68.78
    support: 4700.00
  micro avg:
    precision: 77.88
    recall: 73.28
    f1-score: 75.48
    support: 12800.00
  macro avg:
    precision: 80.48
    recall: 71.15
    f1-score: 74.48
    support: 12800.00
  weighted avg:
    precision: 79.62
    recall: 73.28
    f1-score: 75.42
    support: 12800.00
****************************************
Average results for model camembert over 5 seeds:
  LOC:
    precision: 85.63
    recall: 84.80
    f1-score: 85.17
    support: 5000.00
  ORG:
    precision: 87.04
    recall: 56.13
    f1-score: 68.23
    support: 3100.00
  PER:
    precision: 69.41
    recall: 62.13
    f1-score: 65.44
    support: 4700.00
  micro avg:
    precision: 79.58
    recall: 69.53
    f1-score: 74.18
    support: 12800.00
  macro avg:
    precision: 80.69
    recall: 67.69
    f1-score: 72.95
    support: 12800.00
  weighted avg:
    precision: 80.02
    recall: 69.53
    f1-score: 73.82
    support: 12800.00
****************************************
Average results for model mbert+narabizi over 5 seeds:
  LOC:
    precision: 86.12
    recall: 90.00
    f1-score: 87.93
    support: 5000.00
  ORG:
    precision: 90.64
    recall: 50.32
    f1-score: 64.69
    support: 3100.00
  PER:
    precision: 63.51
    recall: 62.98
    f1-score: 62.47
    support: 4700.00
  micro avg:
    precision: 77.03
    recall: 70.47
    f1-score: 73.43
    support: 12800.00
  macro avg:
    precision: 80.09
    recall: 67.77
    f1-score: 71.69
    support: 12800.00
  weighted avg:
    precision: 78.91
    recall: 70.47
    f1-score: 72.95
    support: 12800.00
****************************************
Average results for model mbert over 5 seeds:
  LOC:
    precision: 80.26
    recall: 85.20
    f1-score: 82.60
    support: 5000.00
  ORG:
    precision: 88.66
    recall: 50.32
    f1-score: 64.15
    support: 3100.00
  PER:
    precision: 67.55
    recall: 60.43
    f1-score: 63.57
    support: 4700.00
  micro avg:
    precision: 76.58
    recall: 67.66
    f1-score: 71.79
    support: 12800.00
  macro avg:
    precision: 78.82
    recall: 65.32
    f1-score: 70.11
    support: 12800.00
  weighted avg:
    precision: 77.63
    recall: 67.66
    f1-score: 71.15
    support: 12800.00
****************************************
Average results for model xlmt over 5 seeds:
  LOC:
    precision: 80.74
    recall: 90.40
    f1-score: 85.19
    support: 5000.00
  ORG:
    precision: 90.78
    recall: 57.42
    f1-score: 70.07
    support: 3100.00
  PER:
    precision: 76.69
    recall: 64.26
    f1-score: 69.76
    support: 4700.00
  micro avg:
    precision: 80.68
    recall: 72.81
    f1-score: 76.49
    support: 12800.00
  macro avg:
    precision: 82.74
    recall: 70.69
    f1-score: 75.01
    support: 12800.00
  weighted avg:
    precision: 81.69
    recall: 72.81
    f1-score: 75.86
    support: 12800.00
****************************************
Average results for model dziribert over 5 seeds:
  LOC:
    precision: 79.28
    recall: 89.60
    f1-score: 84.08
    support: 5000.00
  ORG:
    precision: 85.11
    recall: 58.71
    f1-score: 69.00
    support: 3100.00
  PER:
    precision: 68.45
    recall: 71.06
    f1-score: 69.61
    support: 4700.00
  micro avg:
    precision: 75.88
    recall: 75.31
    f1-score: 75.56
    support: 12800.00
  macro avg:
    precision: 77.61
    recall: 73.12
    f1-score: 74.23
    support: 12800.00
  weighted avg:
    precision: 76.71
    recall: 75.31
    f1-score: 75.12
    support: 12800.00
****************************************
Average results for model characterBertarabizi over 5 seeds:
  LOC:
    precision: 95.67
    recall: 86.40
    f1-score: 90.75
    support: 5000.00
  ORG:
    precision: 89.58
    recall: 52.90
    f1-score: 66.30
    support: 3100.00
  PER:
    precision: 73.06
    recall: 62.98
    f1-score: 66.95
    support: 4700.00
  micro avg:
    precision: 85.24
    recall: 69.69
    f1-score: 76.52
    support: 12800.00
  macro avg:
    precision: 86.10
    recall: 67.43
    f1-score: 74.67
    support: 12800.00
  weighted avg:
    precision: 85.89
    recall: 69.69
    f1-score: 76.09
    support: 12800.00


    % \begin{table*}[!ht]
%     \centering
%     \footnotesize
% \begin{tabular}{lcccccc}
% \toprule
% \multirow{2}{*} & \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test} \\
% \cline{2-7}
% & UPOS & UAS & LAS & UPOS & UAS & LAS \\ \midrule
% mbert & 79.80 \textsuperscript{$\pm$ 0.25} & 67.81 \textsuperscript{$\pm$ 0.23} & 55.42 \textsuperscript{$\pm$ 0.43 }& 80.25 \textsuperscript{$\pm$ 0.45} & 70.41 \textsuperscript{$\pm$ 0.09} & 58.43 \textsuperscript{$\pm$ 0.40} \\
% characterBertarabizi & 78.15 $\pm$ 0.56 & 67.34 $\pm$ 0.55 & 54.24 $\pm$ 0.48 & 78.61 $\pm$ 0.73 & 69.08 $\pm$ 0.36 & 56.42 $\pm$ 0.16 \\
% mbert+narabizi & 84.01 $\pm$ 0.56 & 71.24 $\pm$ 0.36 & 60.03 $\pm$ 0.57 & 84.49 $\pm$ 0.39 & 74.02 $\pm$ 0.35 & 63.12 $\pm$ 0.40 \\
% dziribert & 82.15 $\pm$ 2.01 & 71.31 $\pm$ 0.37 & 60.07 $\pm$ 0.88 & 82.82 $\pm$ 2.22 & 74.05 $\pm$ 0.52 & 62.70 $\pm$ 0.97 \\
% camembert & 69.54 $\pm$ 2.22 & 66.25 $\pm$ 0.49 & 51.78 $\pm$ 0.41 & 71.66 $\pm$ 2.95 & 70.49 $\pm$ 1.06 & 56.01 $\pm$ 1.19 \\
% xlmt & 77.42 $\pm$ 0.87 & 68.24 $\pm$ 0.48 & 55.13 $\pm$ 0.44 & 77.99 $\pm$ 0.94 & 71.29 $\pm$ 0.65 & 57.93 $\pm$ 0.74 \\

% \bottomrule
% \end{tabular}
% \caption{NEW RESULTS UD}
% \end{table*}
% \begin{table*}[!ht]
% \centering
%     \footnotesize
% \begin{tabular}{lccccc}
% \toprule
% \textbf{Model} & \textbf{LOC} & \textbf{ORG} & \textbf{PER} & \textbf{macro avg} \\
% \midrule
% camembert+narabizi & 85.61 & 69.06 & 68.78 & 74.48 \\
% camembert & 85.17 & 68.23 & 65.44  & 67.69 \\
% mbert+narabizi & 87.93 & 64.69 & 62.47 & 71.69 \\
% mbert & 82.60 & 64.15 & 63.57  & 70.11 \\
% xlmt & 85.19 & 70.07 & 69.76 & 75.01\\
% dziribert & 84.08 & 69.00 & 69.61 & 74.23 \\
% characterBertarabizi & 90.75 & 66.30 & 66.955 & 74.67  \\
% \bottomrule
% \end{tabular}
% \caption{NER F1-scores for various models over 5 seeds}
% \label{tab:f1-scores}
% \end{table*}


% \begin{table}[]
%     \centering
%     \footnotesize
% \begin{tabular}{llll}
% \hline
% \multicolumn{2}{c}{NERDz}            & \multicolumn{2}{c}{Our dataset}       \\     
% \midrule
% \multicolumn{1}{l}{Entities} & Count & \multicolumn{1}{l}{Entities} & Count \\     \toprule
% \per                           & 467   & \per                           & 479   \\ 
% GPE/\loc                       & 479   & \loc                           & 466   \\ 
% \org    
% & 290   & \org/\comp                      & 265  \\
%     \bottomrule
% \end{tabular}%
%     \caption{Mapping of NER Labels in Our Dataset to the Published NERDz dataset.}
%     \label{tab:comp-nerdz}
% \end{table}


% fix tokenization problem + fix cycles + add translations + identify duplicates + consistency
% - word splitting on conjunctions, interjections "ya" and determiners and prepositions when next to noun phrases. ex : w
% - determiners : for sun letters, splitting is on the first vowel (a or e), ex : e ssalam, e dounoub.
% - determiners : lemma field is aligned with French translation (e ssalam -> la paix).
% - prepositions : split on first letter+i when possible brabi -> b rabi, fighaet -> fi g haet
% - Determiners and PROPN splitting : need to determine a rule
% - Tool used for splitting: Grew (graph rewriting tool for NLP (Guillaume et al)
%tokenization : 
%normalization des scores (4-0)
%tokenisation des entites nommees + choix d'annotation
%coquilles
%pos tagging :
%gestion de plusieurs langues , ex  tous/tout (fr) , ga3/ koul/koulech (ar dz), jami3an/ajma3in (msa)
%correction bessah et belli qui sont des conjonctions
%dependencies :
%normalization des marqueurs de discours (inshaallah, mashaallah, sws, 1 2 3 viva l'algerie, vocatifs)
%repérage et normalisation de constructions spécifiques (ex : hada hiya el korra, dislocated ...).
%traduction :
%prise en compte des locutions/ idiomes dans la traduction (ex : betna fi ermel, skara + fi , madabiya ...)
% Tool used for consistency check : Errator (to cite)



% \paragraph{Why transfer learning with Maltese?}
% Maltese is the national language of Malta, a small island country in the Mediterranean Sea. It is a Semitic language that is closely related to Arabic and Hebrew. Maltese is written with the Latin script and includes some unique letters that are not found in other languages, such as \iffalse ċ, ġ, ħ, and ż\else to replace by macros \fi. Maltese has a long and rich history, and various languages, including Arabic, Italian, English, and French, have influenced it.
% % to do add citation
% Maltese is similar to North African languages in its grammar and syntax. Like other Semitic languages, Maltese has a noun and verb inflection system that involves changing the form of words to indicate their role in the sentence. This is similar to the grammatical system used in North African languages.
% Moreover, Maltese has borrowed many words from Arabic, including several words shared with other North African languages. For example, Maltese and North African languages both use the word \iffalse "għar"\else ghar \fi to mean "house" and the word \iffalse "ħabib" \else habib \fi to mean "friend."
% Maltese has many similarities with North African languages due to its shared Semitic heritage and linguistic and cultural exchange history with North Africa.

% I run experiments using deprel accuracy as the metric to choose the best models but I got same tendencies as with head accuracy (results comments bellow)

% Results for mbert:
% Mean UPOS score on Test: 78.83 +/- 1.33
% Mean UAS score on Test: 70.74 +/- 0.57
% Mean LAS score on Test: 58.12 +/- 0.81

% Results for characterBertarabizi:
% Mean UPOS score on Test: 77.75 +/- 3.23
% Mean UAS score on Test: 68.73 +/- 0.67
% Mean LAS score on Test: 56.04 +/- 0.52

% Results for dziribert:
% Mean UPOS score on Test: 82.31 +/- 1.11
% Mean UAS score on Test: 74.01 +/- 0.80
% Mean LAS score on Test: 62.43 +/- 0.68

%     Training model 1
% Number of SpaceAfter=No features in gold data: 129
% Tokenizer tokens - system: 3558, gold: 3616, precision: 96.54%, recall: 94.99%, f1: 95.76%
% Tokenizer multiword tokens - system: 95, gold: 251, precision: 78.95%, recall: 29.88%, f1: 43.35%
% Tokenizer words - system: 3654, gold: 3882, precision: 91.71%, recall: 86.32%, f1: 88.93%

% Training model 2
% Number of SpaceAfter=No features in gold data: 134
% Tokenizer tokens - system: 3692, gold: 3761, precision: 96.89%, recall: 95.11%, f1: 95.99%
% Tokenizer multiword tokens - system: 92, gold: 240, precision: 86.96%, recall: 33.33%, f1: 48.19%
% Tokenizer words - system: 3786, gold: 4013, precision: 93.05%, recall: 87.79%, f1: 90.34%

% Training model 3
% Number of SpaceAfter=No features in gold data: 127
% Tokenizer tokens - system: 3591, gold: 3649, precision: 97.35%, recall: 95.81%, f1: 96.57%
% Tokenizer multiword tokens - system: 83, gold: 211, precision: 80.72%, recall: 31.75%, f1: 45.58%
% Tokenizer words - system: 3675, gold: 3874, precision: 93.61%, recall: 88.80%, f1: 91.14%

% Training model 4
% Number of SpaceAfter=No features in gold data: 123
% Tokenizer tokens - system: 3804, gold: 3856, precision: 97.50%, recall: 96.19%, f1: 96.84%
% Tokenizer multiword tokens - system: 116, gold: 243, precision: 78.45%, recall: 37.45%, f1: 50.70%
% Tokenizer words - system: 3923, gold: 4113, precision: 93.27%, recall: 88.96%, f1: 91.07%


% Training model 5
% Number of SpaceAfter=No features in gold data: 143
% Tokenizer tokens - system: 3608, gold: 3679, precision: 97.23%, recall: 95.35%, f1: 96.28%
% Tokenizer multiword tokens - system: 110, gold: 221, precision: 73.64%, recall: 36.65%, f1: 48.94%
% Tokenizer words - system: 3719, gold: 3911, precision: 92.98%, recall: 88.42%, f1: 90.64%
